Expressiveness and Decidability of Temporal Logics for Asynchronous Hyperproperties

Hyperproperties are properties of systems that relate different executions traces, with many applications from security to symmetry, consistency models of concurrency, etc. In recent years, different linear-time logics for specifying asynchronous hyperproperties have been investigated. Though model checking of these logics is undecidable, useful decidable fragments have been identified with applications e.g. for asynchronous security analysis. In this paper, we address expressiveness and decidability issues of temporal logics for asynchronous hyperproperties. We compare the expressiveness of these logics together with the extension S1S[E] of S1S with the equal-level predicate by obtaining an almost complete expressiveness picture. We also study the expressive power of these logics when interpreted on singleton sets of traces. We show that for two asynchronous extensions of HyperLTL, checking the existence of a singleton model is already undecidable, and for one of them, namely Context HyperLTL (HyperLTL_C), we establish a characterization of the singleton models in terms of the extension of standard FO[<] over traces with addition. This last result generalizes the well-known equivalence between FO[<] and LTL. Finally, we identify new boundaries on the decidability of model checking HyperLTL_C.

==> UndecidabilityDHS.tex <==
\section{Undecidability results}\label{sec:undecidability}

In this section, we establish that both model-checking and homogeneous satisfiability for the novel logic $\DHS$, and in particular, for the fragment
$\DHS(A,B)$, are undecidable  by a polynomial-time reduction
from the \emph{halting problem for Minsky $2$-counter machines}~\cite{Minsky67}.



\begin{theorem}\label{theorem:undecidability}
Model-checking and homogeneous satisfiability for $\DHS(A,B)$ are undecidable even for the following fragments:
\begin{compactitem}
  \item the fragment $\DHS_X(A,B)$ for each $X\in\{A,B\}$ even if, additionally, equality constraints are disallowed;
  \item the fragment L/U of $\DHS(A,B)$ even if, additionally, one assume that non-trivial constraints are lower-bounds and are associated
  only to the existential modalities in the \PNF\ of the given L/U $\DHS(A,B)$ formula.
\end{compactitem}
\end{theorem}
\begin{proof}
Recall that a  nondeterministic Minsky $2$-counter machine is a tuple $M = \tpl{Q,q_\init,q_\halt,  \Delta}$,
where  $Q$ is a finite set of (control) locations, $q_\init\in Q$ is the initial location,   $q_\halt\in Q$ is the halting location, and
   $\Delta \subseteq Q\times \Inst \times Q$ is a transition relation over the instruction set $\Inst= \{\inc,\dec,\zero\}\times \{1,2\}$.
For a transition $\delta=(q,\instr,q')\in \Delta$, we
define $\From(\delta):= q$, $\instr(\delta):=\instr$,
and $\To(\delta):= q'$.
Without loss of generality we assume that:
\begin{itemize}
  \item for each transition $\delta\in \Delta$, $\From(\delta)\neq q_\halt$ and $\To(\delta )\neq q_\init$, and
    \item there is exactly one transition in $\Delta$, denoted $\delta_\init$, having as source %the initial
    location $q_\init$.
\end{itemize}

An $M$-configuration is a pair $(q,\nu)$ consisting of a location $q\in Q$ and a counter valuation $\nu: \{1,2\}\to \Nat$.
A  computation of $M$ is a non-empty \emph{finite} sequence $(q_1,\nu_1),\ldots ,(q_k,\nu_k)$ of configurations such that for all $1\leq i<k$, there is
some instruction $\instr_i=(\ttag_i,c_i)\in \Inst$  so that $(q_i,\instr_i,q_{i+1})\in \Delta$ and:
%
  (i)    $\nu_{i+1}(c)= \nu_i(c)$ if   $c\neq c_i$;
  (ii)  $\nu_{i+1}(c_i)= \nu_i(c_i) +1$ if $\ttag_i = \inc$;
  (iii) $\nu_{i+1}(c_i)= \nu_i(c_i) -1$ and $\nu_i(c_i)>0$ if $\ttag_i = \dec$; and
   (iv)  $\nu_{i+1}(c_i)= \nu_i(c_i)=0$ if $\ttag_i =\zero$.
%
The halting problem is to decide whether for a machine $M$, there is a computation starting at the \emph{initial}
configuration $(q_\init, \nu_\init)$, where $\nu_\init(1) = \nu_\init(2) = 0$,
and leading to some
halting configuration
$(q_{\halt}, \nu)$ (it was proved to be undecidable in~\cite{Minsky67}).

We first prove Theorem~\ref{theorem:undecidability} for the part concerning the model-checking problem. We construct a finite Kripke structure
$\Ku_M$ and a $\DHS(A,B)$ formula $\varphi_M$ in each of the indicated fragments in Theorem~\ref{theorem:undecidability} such that
$M$ halts \emph{if and only if} there exists an initial infinite path $\pi$ of $\Ku_M$ whose trace satisfies $\varphi_M$
\emph{if and only if} $\Ku_M$ is not a model of $\neg \varphi_M$. Then, at the end of the proof, we show how the construction can be
easily modified for obtaining a reduction from the halting problem to homogeneous satisfiability.


We exploit the set $\Prop$ of atomic proposition defined as
%
\[
\Prop:=V_\Delta\times \{\Beg, \End,1_L,1_R,2_L,2_R,[_L,]_L,[_R,]_R\}
\]
 where
$V_\Delta$  is the set of pairs $(\delta'_\bot,\delta)$ such that $\delta'_\bot\in\Delta\cup\{\bot\}$,
$\delta\in\Delta$, and $\To(\delta'_\bot)=\From(\delta)$ if $\delta'_\bot\neq\bot$, and $\delta=\delta_\init$ otherwise. Intuitively, in the pair $(\delta'_\bot,\delta)$,
$\delta$ represents the transition currently taken by $M$ from the current non-halting configuration $C$, while
$\delta'_\bot$ is $\bot$ if $C$ is the initial configuration, and $\delta'$ represents the transition exploited by $M$ in the previous computational step otherwise.

A configuration $C=(q,\nu)$ of $M$ is encoded by  finite words  $w_C$ over $2^{\Prop}$ (\emph{configuration codes}) of length $10+2\cdot\nu(1)+2\cdot\nu(2)$  illustrated in the following figure, where $v\in V_\Delta$ (called \emph{$V_\Delta$-value of $w_C$}) is of the form $(\delta'_\bot,\delta)$ such that $\From(\delta)=q$.
\input{EncodingStrongMinimal.tex}
Note that the configuration code $w_C$ is subdivided in two parts. In the left part (resp., right part), the encoding of
counter $1$ (resp., $2$) precedes the encoding of counter $2$ (resp., $1$).
The value $\nu(1)$   of counter $1$  is encoded by the length, which is $\nu(1)+1$, of the subword $\{v,1_L\}^{\nu(1)+1}$ (we call \emph{$1_L$-counter cycle})    marked by $1_L$ in the left part, and the subword $\{v,1_R\}^{\nu(1)+1}$ (we call \emph{$1_R$-counter cycle})  marked by  $1_R$ in the right part, and similarly for counter $2$. The first (resp., last) position of $w_c$ is marked by $\Beg$ (resp., $\End$). Finally,
the  four positions marked by $[_L$, $]_L$, $[_R$, and $]_R$, respectively, are called \emph{tagged} positions:
they are used to check by $\DHS(A,B)$ formulas that increment and decrement $M$-instructions are correctly encoded. Moreover, we require that the configuration code $w_C$ satisfies the following additional requirement (\emph{$V_\Delta$-requirement}), with  $v=(\delta'_\bot,\delta)$ and $\delta=(q,\instr,q')$:
\begin{itemize}
  \item if $\delta=\delta_\init$ then the counter cycles have length $1$  (\emph{initialization});
  \item if $\instr=(\dec,c)$ (resp., $\instr=(\zero,c)$), then the counter cycles marked by $c_L$ and $c_R$ are greater than $1$ (resp., are equal to $1$).
\end{itemize}

A \emph{pseudo-configuration code} is defined as a configuration code but the
lengths of the counter cycles  are arbitrary with the restriction that the $V_\Delta$-requirement is fulfilled. In particular, in a pseudo-configuration code, the requirement that for each counter $c\in \{1,2\}$, the length of the counter cycle marked by $c_L$ coincides with the length of the counter cycle marked by $c_R$ is relaxed.

A \emph{pseudo-computation code}  $w_M$ is an infinite word over $2^{\Prop}$ of the form $w_M=w_0  \cdots  w_n \cdot \{\Beg\} \cdot \emptyset^{\omega}$ for some $n\geq 0$ such that
\begin{compactitem}
  \item[(i)] $w_i$ is
a \emph{pseudo-configuration code} for all $0\leq i\leq n$,
  \item[(ii)] for all $0\leq i<n $, the second component of the $V_\Delta$-value of  $w_i$ coincides
  with the first component of the $V_\Delta$-value of  $w_{i+1}$ (\emph{consecution});
  \item[(ii)]  the $V_\Delta$-value of   $\pi_0$ is
$(\bot,\delta_\init)$ (\emph{initialization}),
  \item[(iv)] the $V_\Delta$-value of $\pi_n$ is of the form $(\delta'_\bot,\delta)$ such that $\To(\delta)=q_\halt$ (\emph{halting}).
\end{compactitem}\vspace{0.1cm}

By construction, we easily deduce the following result.\vspace{0.1cm}

\noindent \textbf{Claim.} One can construct in polynomial-time  a finite Kripke structure $\Ku_M$ over $\Prop$ satisfying the following:
the set of traces associated with the initial infinite paths of $\Ku_M$ which visit some state with empty label coincides
with the set of pseudo-computation codes. \vspace{0.1cm}


By the previous claim, for capturing the  traces of the initial infinite paths of $\Ku_M$  representing all and only the pseudo-computation codes it suffices to exploit the following $\HS(A,B)$ formula $\varphi_\emptyset$ (i.e., a formula in the unconstrained fragment of $\DHS(A,B)$):
\[
\varphi_\emptyset:=\hsA \hsA (\Length_1 \wedge \displaystyle{\bigwedge_{p\in\Prop}}\neg p)
\]
%
where  $\Length_1 := \hsUB \false$  characterizes the intervals of length $1$.

For each instruction $\instr\in \{\inc,\dec,\zero\}\times \{1,2\}$ of the machine $M$, let $V_\instr$ be the subset of $V_\Delta$ consisting of the pairs $(\delta'_\bot,\delta)$ such that $\delta'_\bot\neq \bot$ and $\instr(\delta'_\bot)=\instr$.
We now consider the crucial part of the reduction consisting in defining $\DHS(A,B)$ formulas guaranteing that along a pseudo-computation code $w_M$
the following holds:
\begin{compactitem}
\item for each pseudo-configuration code of $w_M$, the lengths of the left and right counter-cycles for counter $1$ (resp., $2$) coincide (\emph{left-right requirement}), and
  \item the lengths of the counter cycles in the non-initial pseudo-configuration codes of $w_M$
whose $V_\Delta$-values are in $V_\instr$
  are updated consistently with the instruction $\instr$ (\emph{$\instr$-requirement}).
\end{compactitem}\vspace{0.1cm}

In order to capture the previous requirements, we first define some auxiliary (unconstrained) $\HS(A,B)$ formulas.
For all tags $\Tag,\Tag'\in \{\Beg, \End,1_L,1_R,2_L,2_R,[_L,]_L,[_R,]_R\}$, we define an $\HS(A,B)$ formula $\varphi(\Tag,\Tag')$ capturing the non-singular intervals, if any,
along a pseudo-computation code whose start point (resp., ending point) is marked by $\Tag$ (resp., $\Tag'$), and each internal point is not marked by a tag in $\{\Tag,\Tag'\}$:
\[
\varphi(\Tag,\Tag')::= \neg\Length_1\wedge \hsB(\Length_1\wedge \Tag)\wedge \hsA(\Length_1\wedge \Tag') \wedge \hsUB (\neg\Length_1 \rightarrow \hsUA (\neg\Tag \wedge \neg\Tag'))
\]
For instance, the formula $\varphi(\Beg,\End)$ is fulfilled by an interval (infix subword) along a pseudo-computation code iff
the interval corresponds to a pseudo-configuration code. As another example, the formula $\varphi(\Beg,]_L)$ captures the left parts of pseudo-configuration codes
along a pseudo-computation code. \vspace{0.2cm}

\noindent\emph{Expressing the left-right requirement.} Our encoding ensures that the left-right requirement is fulfilled along a pseudo-computation code $w_M$ if and only if:
\begin{compactitem}
  \item for each interval $I$ of $w_M$ satisfying $\varphi(\Beg,\End)$, the length of the unique prefix of $I$ leading to the position marked by $]_L$ is the half of $I$
  (this ensures that along pseudo-configuration codes, the left and right parts have the same length);
  \item for each interval $I$ of $w_M$ satisfying $\varphi([_L,]_R)$, the length of the unique prefix of $I$ leading to the position marked by $]_L$ is the half of $I$
  (this ensures that along a pseudo-configuration code, the left and right counter-cycles for counter $2$ have the same length).
\end{compactitem}\vspace{0.1cm}

A $\DHS_B(A,B)$ formula $\varphi_B$ without equality constraints ensuring the previous requirements can be defined as follows:
%
\[
\begin{array}{ll}
  \varphi_B ::=  &  \hsUA \hsUA \bigl[\varphi(\Beg,\End) \rightarrow ( \neg \hsB_{< \frac{1}{2}} \varphi(\Beg,]_L)  \wedge \neg \hsB_{> \frac{1}{2}} \varphi(\Beg,]_L)) \,\wedge \\
    & \phantom{\hsUA \hsUA \bigl(}  \varphi([_L,]_R) \rightarrow ( \neg \hsB_{< \frac{1}{2}} \varphi([_L,]_L)  \wedge \neg \hsB_{> \frac{1}{2}} \varphi([_L,]_L))\bigr]
\end{array}
\]
%
A $\DHS_A(A,B)$ formula $\varphi_A$ without equality constraints expressing the same requirements can be instead defined as follows:
%
\[
\begin{array}{ll}
  \varphi_A ::=  &  \hsUA \hsUA \bigl[\varphi(\Beg,[_R) \rightarrow ( \neg \hsA_{< 1} \varphi([_R,\Beg)  \wedge \neg \hsA_{> 1} \varphi([_R,\Beg)) \,\wedge \\
    & \phantom{\hsUA \hsUA \bigl(}  \varphi([_L,[_R) \rightarrow ( \neg \hsA_{< 1} \varphi([_R,1_R)  \wedge \neg \hsA_{> 1} \varphi([_R,1_R))\bigr]
\end{array}
\]
%
Finally an L/U $\DHS(A,B)$ formula $\varphi_{L/U}$ satisfying the left-right requirement is given by:
 %
\[
\begin{array}{ll}
  \varphi_{L/U} ::=  &  \hsUA \hsUA \bigl[(\varphi(\Beg,\End) \rightarrow \hsB_{\leq \frac{1}{2}} \varphi(\Beg,]_L)
                                           \wedge (\varphi(\Beg,[_R) \rightarrow  \hsA_{\leq 1} \varphi([_R,\Beg)) \,\wedge \\
    & \phantom{\hsUA \hsUA \bigl(} (\varphi([_L,]_R) \rightarrow  \hsB_{\leq \frac{1}{2}} \varphi([_L,]_L)) \wedge
                                   (\varphi([_L,[_R) \rightarrow   \hsA_{\leq 1} \varphi([_R,1_R))\bigr]
\end{array}
\]
%
Note that the non-trivial constraints in $\varphi_{L/U}$ are only lower bounds and are associated to the existential temporal modalities in the
\PNF\ of $\varphi_{L/U}$.\vspace{0.1cm}

\noindent\emph{Expressing the $\instr$-requirement for $\instr\in \{\inc,\zero,\dec\}\times \{1,2\}$.}
Let $w_M$ be a pseudo-computation code, $w_C$
a  non-initial pseudo-configuration code  of $w_M$ with $V_\Delta$-value  in $V_\instr$, and $n_1$ and $n_2$
 the values of counters $1$ and $2$ in the right part of the
pseudo-configuration code $w_{C_p}$ preceding $w_C$ along $w_M$ (i.e., the lengths of counter cycles in $w_{C_p}$ marked by $1_R$ and $2_R$ minus one).
Here, we focus on the case   where $\instr=(\dec,2)$  (the cases of decrement instructions of counter $1$ and zero-test and increment instructions being similar). We need to ensure that $n'_1= n_1$ and $n'_2 = n_2-1$, where $n'_1$ and $n'_2$ are the values of counters $1$ and $2$ in the left part of $w_C$.
For this, we crucially exploit the fact that the encoding of counter~$1$ in the left part of $w_C$ is preceded by the encoding of counter $1$ in the right part of $w_{C_p}$ (as illustrate in the figure below). Thus, by construction, it suffices to require that
\begin{compactitem}
  \item for each interval $I$ of $w_M$ satisfying $\varphi(]_R,[_L)$ whose endpoint has a $V_\Delta$-value  in $V_\instr$, the length of the unique prefix of $I$ leading to the position marked by $\End$ is the half of $I$
  (this ensures that $n'_1=n_1$);
  \item for each interval $I$ of $w_M$ satisfying $\varphi([_R,[_R)$ whose endpoint has a $V_\Delta$-value  in $V_\instr$, the length of the unique prefix of $I$ leading to the position marked by $\End$ is the half of $I$
  (this ensures that $n'_1+n'_2= n_1+n_2-1$).
\end{compactitem}\vspace{0.1cm}

For all tags $\Tag,\Tag'\in \{\Beg, \End,1_L,1_R,2_L,2_R,[_L,]_L,[_R,]_R\}$, let $\varphi_{\instr}(\Tag,\Tag')$ be the $\HS(A,B)$ formula
defined as  $\varphi_{\instr}(\Tag,\Tag'):= \varphi(\Tag,\Tag')\wedge \hsA(\Length_1 \wedge \bigvee_{v\in V_\instr} v)$.
\input{EncodingStrongMinimalConsecutio.tex}

Here, we  define a $\DHS_B(A,B)$ formula $\varphi^{B}_{\instr}$ without equality constraints ensuring the previous requirements.
The definitions of a $\DHS_A(A,B)$ formula and an L/U formula $\DHS(A,B)$  ensuring the same requirements follow a pattern similar to that illustrated
for the left-right requirement.
%
\[
\begin{array}{ll}
  \varphi^{B}_{\instr} ::=  &  \hsUA \hsUA \bigl[\varphi_{\instr}(]_R,[_L) \rightarrow ( \neg \hsB_{< \frac{1}{2}} \varphi(]_R,\End)  \wedge \neg \hsB_{> \frac{1}{2}} \varphi(]_R,\End)) \,\wedge \\
    & \phantom{\hsUA \hsUA \bigl(}  \varphi_{\instr}([_R,[_R) \rightarrow ( \neg \hsB_{< \frac{1}{2}} \varphi([_R,\End)  \wedge \neg \hsB_{> \frac{1}{2}} \varphi([_R,\End))\bigr]
\end{array}
\]
%
Finally, for the reduction to homogenous satisfiability, it suffices to observe that one can easily construct an (unconstrained) $\HS(A,B)$ capturing the pseudo-computation codes. This conclude the proof of Theorem~\ref{theorem:undecidability}.
\end{proof}


